GraphMI: Extracting Private Graph Data from Graph Neural Networks

As machine learning becomes more widely used for critical applications, the need to study its implications in privacy turns to be urgent. Given access to the target model and auxiliary information, the model inversion attack aims to infer sensitive features of the training dataset, which leads to great privacy concerns. Despite its success in grid-like domains, directly applying model inversion techniques on non-grid domains such as graph achieves poor attack performance due to the difficulty to fully exploit the intrinsic properties of graphs and attributes of nodes used in Graph Neural Networks (GNN). To bridge this gap, we present \textbf{Graph} \textbf{M}odel \textbf{I}nversion attack (GraphMI), which aims to extract private graph data of the training graph by inverting GNN, one of the state-of-the-art graph analysis tools. Specifically, we firstly propose a projected gradient module to tackle the discreteness of graph edges while preserving the sparsity and smoothness of graph features. Then we design a graph auto-encoder module to efficiently exploit graph topology, node attributes, and target model parameters for edge inference. With the proposed methods, we study the connection between model inversion risk and edge influence and show that edges with greater influence are more likely to be recovered. Extensive experiments over several public datasets demonstrate the effectiveness of our method. We also show that differential privacy in its canonical form can hardly defend our attack while preserving decent utility.

==> defense.tex <==
\section{Defense for GMI attack}

One of the most popular countermeasure against privacy attack is differential privacy (DP). Its definition is based on the idea that if two databases differ only by one record and are used by the same algorithm, the output of that algorithm should be similar. More formally:
\begin{myDef}
    (($\epsilon,\delta$)-differential privacy) A randomized mechanism $\mathcal{M}$ with domain $\mathcal{R}$ and output $\mathcal{S}$ satisfies ($\epsilon,\delta$)-differential privacy if for any neighboring  datasets $D, D' \in \mathcal{R}$, which differ by at most one record and for any subsets of outputs $S$ it holds that:
\begin{equation}
    Pr[\mathcal{M}(D)\in S]\le e^{\epsilon}Pr[\mathcal{M}(D')\in S]+\delta,
\end{equation}
\end{myDef}
\noindent where $\epsilon$ is the privacy budget and $\delta$ is the failure probability.\par
\begin{figure}[!t]
	\centering
	\includegraphics[width=0.47\textwidth]{figs/illustration2.pdf}
	\caption{Defense based on graph preprocessing}
	\label{illustration2}
\end{figure}
Differential privacy is one general approach for protecting privacy. However, it is not designed for graph, especially for graph model inversion attack. Here we propose one simple defense method based on graph preprocessing (summarized in algorithm 2). Instead of adding noise in GNN model training, our method adds pseudo edges in the training graph to "hide" real edges from model inversion. Specifically, to preserve utility of trained GNN model, we add pseudo edges with high feature similarity (Figure~\ref{illustration2}). Compared with convolutional neural networks for image data, graph neural network generally has fewer layers and parameters. GNN models essentially aggregate features according to graph structure. Previous work on graph adversarial learning~\cite{wu2019adversarial} suggests that adding edges with low feature similarity will severely undermines the utility of GNN model in node classification. Compared with adding edges randomly in the training graph, adding edges with high feature similarity helps preserve utility. 
\begin{algorithm}[h]
  \caption{Defense for GMI attack based on graph preprocessing}
  \begin{algorithmic}[1]
    \Require
      Training graph adjacency matrix $A$;
      Feature vectors $x_i$;
      Edge selection threshold $t$;
    \Ensure
      Trained GNN model, $f$;
      
    \State Normalize feature vectors $x_i$
    \State Calculate similarity matrix $S$
    \For{all entries in $A$}
      \If {$S_{ij}\textgreater t$ and $A_{ij}=0$}
      \ThenApply Set $A_{ij}=1$
      \EndIf
    \EndFor
    \State Train GNN model on $A$
    \label{code1}
  \end{algorithmic}
\end{algorithm}
%
